Gradient Importance Sampling

Adaptive Monte Carlo schemes developed over the last years usually seek to ensure ergodicity of the sampling process in line with MCMC tradition. This poses constraints on what is possible in terms of adaptation. In the general case ergodicity can only be guaranteed if adaptation is diminished at a certain rate. Importance Sampling approaches offer a way to circumvent this limitation and design sampling algorithms that keep adapting. Here I present a gradient informed variant of SMC (and its special case Population Monte Carlo) for static problems.

==> greektex.tex <==
\let\mathbbm=\mathbb

\let\textGamma=\Gamma
\let\textDelta=\Delta
\let\textEpsilon=\Epsilon
\let\textZeta=\Zeta
\let\textEta=\Eta
\let\textTheta=\Theta
\let\textIota=\Iota
\let\textKappa=\Kappa
\let\textLambda=\Lambda
\let\textMu=\Mu
\let\textNu=\Nu
\let\textXi=\Xi
\let\textOmicron=\Omicron
\let\textPi=\Pi
\let\textRho=\Rho
\let\textSigma=\Sigma
\let\textTau=\Tau
\let\textUpsilon=\Upsilon
\let\textPhi=\Phi
\let\textChi=\Chi
\let\textPsi=\Psi
\let\textOmega=\Omega

\let\textalpha=\alpha
\let\textbeta=\beta
\let\textgamma=\gamma
\let\textdelta=\delta
\let\textepsilon=\epsilon
\let\textzeta=\zeta
\let\textEta=\eta
\let\texttheta=\theta
\let\textiota=\iota
\let\textkappa=\kappa
\let\textlambda=\lambda
\let\textmu=\mu
\let\textnu=\nu
\let\textxi=\xi
\let\textomicron=\omicron
\let\textpi=\pi
\let\textrho=\rho
\let\textsigma=\sigma
\let\textvarsigma=\varsigma
\let\texttau=\tau
\let\textupsilon=\upsilon
\let\textphi=\phi
\let\textchi=\chi
\let\textpsi=\psi
\let\textomega=\omega
